WatME: Towards Lossless Watermarking Through Lexical Redundancy

Text watermarking has emerged as a pivotal technique for identifying machine-generated text. However, existing methods often rely on arbitrary vocabulary partitioning during decoding to embed watermarks, which compromises the availability of suitable tokens and significantly degrades the quality of responses. This study assesses the impact of watermarking on different capabilities of large language models (LLMs) from a cognitive science lens. Our finding highlights a significant disparity; knowledge recall and logical reasoning are more adversely affected than language generation. These results suggest a more profound effect of watermarking on LLMs than previously understood. To address these challenges, we introduce Watermarking with Mutual Exclusion (WatME), a novel approach leveraging linguistic prior knowledge of inherent lexical redundancy in LLM vocabularies to seamlessly integrate watermarks. Specifically, WatME dynamically optimizes token usage during the decoding process by applying a mutually exclusive rule to the identified lexical redundancies. This strategy effectively prevents the unavailability of appropriate tokens and preserves the expressive power of LLMs. We provide both theoretical analysis and empirical evidence showing that WatME effectively preserves the diverse capabilities of LLMs while ensuring watermark detectability.

==> tab/gsm8k_result.tex <==
\begin{table*}[!t]
\setlength{\tabcolsep}{3.55mm}
\centering
\begin{tabular}{lcccccc}
\hline
\multirow{2}{*}{\bf Model} & \multicolumn{2}{c}{delta=3} & \multicolumn{2}{c}{delta=4} & \multicolumn{2}{c}{delta=5} \\
\cline{2-3} \cline{4-5} \cline{6-7} 
 & Accuracy & AUROC & Accuracy & AUROC & Accuracy & AUROC \\
\hline
\textsc{Original} & 11.22\% & - & 11.22\% & - & 11.22\% & - \\
\textsc{Watermark} & 6.67\% & 0.9037 & 6.52\% & 0.9697 & 6.29\% & 0.9947 \\
\textsc{X-Mark} & 10.31\% & 0.9124 & 7.58\% & 0.9719 & 4.55\% & 0.9886 \\
\hline
\end{tabular}
\caption{Performance of Llama2-7B on GSM8K: Comparison of the original model with versions incorporating Vanilla and X-Mark watermarks, under gamma=0.3 and with varying watermark intensities (delta=2,3,4,5).}
\label{tab:my_label}
\end{table*}




==> tab/human_eval.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{0.7mm}
\small
\centering
\begin{tabular}{l|ccc}
\toprule
\textbf{Method} & Semantic. & Contextual. & grammatical. \\

\midrule
Dictionary-based & 1.40 & 1.27 & 1.26  \\

\midrule
Prompting-based & 1.28 & 1.34 & 1.35  \\

\bottomrule
\end{tabular}
\caption{\label{tab:human_eval} Human evaluation for the quality of clusters mined by different methods. 
}

\end{table}


==> tab/truthfulqa_result.tex <==
\begin{table*}[!t]
\small
\centering
\setlength{\tabcolsep}{0.05mm}
\begin{tabular}{c*{12}{S}}
\toprule
\multirow{2}{*}{\bf Model} & \multicolumn{4}{c}{\thead{delta=3}} & \multicolumn{4}{c}{\thead{delta=4}} & \multicolumn{4}{c}{\thead{delta=5}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
 & {True} & {Info} & {True*Info}  & {AUROC} & {True} & {Info} & {True*Info} & {AUROC} & {True} & {Info} & {True*Info} & {AUROC} \\
\midrule
\multicolumn{1}{c}{\textbf{\textsc{Original}}} & & & & & & & & & & & & \\ 
\multicolumn{1}{c}{\textbf{\textsc{Watermark}}} & 56.30\%	& 74.66\% & 42.03\% & 0.7425 & 55.57\% & 83.84\%	& 46.59\% & 0.8416 & 55.94\% & 85.19\% & 47.66\% & 0.9186 \\ 
\multicolumn{1}{c}{\textbf{\textsc{X-Mark}}} & & & & & & & & & & & & \\ 
\bottomrule
\end{tabular}
\caption{Performance of Llama2-7B on TruthfulQA: Comparison of the original model with versions incorporating Vanilla and X-Mark watermarks, under gamma=0.3 and with varying watermark intensities (delta=2,3,4,5).}
\label{tab:my_label}
\end{table*}
